Modular forms and an explicit Chebotarev variant of the Brun-Titchmarsh theorem

We prove an explicit Chebotarev variant of the Brun--Titchmarsh theorem. This leads to explicit versions of the best-known unconditional upper bounds toward conjectures of Lang and Trotter for the coefficients of holomorphic cuspidal newforms. In particular, we prove that $$\lim_{x \to \infty} \frac{\#\{1 \leq n \leq x \mid \tau(n) \neq 0\}}{x} > 1-1.15 \times 10^{-12},$$ where $\tau(n)$ is Ramanujan's tau-function. This is the first known positive unconditional lower bound for the proportion of positive integers $n$ such that $\tau(n) \neq 0$.

==> 6-BQF.tex <==
Recall that $Q(X, Y)$ is a positive-definite primitive binary integral quadratic form with discriminant $-D$, and let $K = \mathbb{Q}(\sqrt{-D})$. Let $L$ be the Hilbert class field of $K$ and let $F = \mathbb{Q}$; the extension $L/F$ is dihedral of degree $2h(-D)$. Recall also that $p$ is represented by $Q(X, Y)$ precisely when there is a prime ideal $\mathfrak{p}$ of norm $p$ and $\mathfrak{p}$ is in the ideal class corresponding to $Q(X, Y)$. This means that $p$ splits completely in $K$ and for some $\mathfrak{p} \mid p$, $\Frob_\mathfrak{p}$ lies in a prescribed conjugacy class of $\Gal(L/K) \simeq \Cl_K$, and this class is singleton since $L/K$ is abelian. Denote the single element of this class by $\sigma$, which corresponds to $Q(X, Y)$ under the Artin map. So, the condition is that for some $\mathfrak{p} \mid p$, $\Frob_\mathfrak{p} = \{\sigma\}$.

The condition that $p$ splits completely in $K$ is equivalent to the condition that $\Frob_p$ --as an element of $\Gal(K/F)$-- is trivial in $\Gal(K/F)$ or that $\Frob_p$ --as a conjugacy class of $\Gal(L/F)$-- fixes $K$. Since $K$ is an imaginary quadratic field, by \cite[Lemma 9.3]{cox13} we have that
\begin{equation}
    \Gal(L/F) = \Gal(L/K) \rtimes \mathbb{Z}/2\mathbb{Z},
\end{equation}
where the nontrivial element of $\mathbb{Z}/2\mathbb{Z}$ acts on $\Gal(L/K)$ by sending $\sigma$ to $\sigma^{-1}$, and is compatible (via the Artin map) with the $\Gal(K/F)$-action on prime ideals of $K$. So, as a conjugacy class $\Frob_p$ is of the form $\{\tau, \tau^{-1}\}$ for some $\tau \in Gal(L/K)$. When $\N\mathfrak{p} = p$, $\Frob_\mathfrak{p}$ is the unique element of $\Gal(L/K)$ sending $x$ to $x^p$ mod $\mathfrak{P}$ for all $\mathfrak{P}\mid \mathfrak{p}$ where $\mathfrak{P}$ is a prime of $L$, which since $\mathfrak{p}$ and its $\Gal(K/F)$-conjugate lie over $p$, is either $\tau$ or $\tau^{-1}$ in $\Frob_p$. 

So, our condition that $\Frob_\mathfrak{p} = \{\sigma\}$ for some $\mathfrak{p} \mid p$ is equivalent to the condition that for any $\mathfrak{p} \mid p$ (there are two such prime ideals, and they are $\Gal(K/F)$-conjugates), $\Frob_\mathfrak{p} = \sigma$ or $\sigma^{-1}$, and this is further equivalent to $\Frob_p = \{\sigma, \sigma^{-1}\}$ as a conjugacy class of $\Gal(L/F)$. So, $p$ is represented by $Q(X, Y)$ if and only if $\Frob_p = \{\sigma, \sigma^{-1}\}$. By the identification of binary quadratic forms with $\Cl_K$ \cite[Theorem 3.9]{cox13}, $Q(X, Y)$ is properly equivalent to its opposite if and only if $\sigma = \sigma^{-1}$, so $\# \Frob_p= 1$ if $Q(X, Y)$ is properly equivalent to its opposite and $\#\Frob_p = 2$ otherwise. We then apply \cref{thm: BT general} to the Galois tower $L/K/F$ with $G = Gal(L/F)$ and $C$ the conjugacy class containing $\sigma$. To compute the range given by \cref{thm: bqf-main-theorem}, set $n_K = 2$ and $\mathcal{Q}(L/K) = 1$, since the conductor of the Hilbert class field of $K$ is $\mathcal{O}_K$.

